High Order Accurate Hermite Schemes on Curvilinear Grids with Compatibility Boundary Conditions

High order accurate Hermite methods for the wave equation on curvilinear domains are presented. Boundaries are treated using centered compatibility conditions rather than more standard one-sided approximations. Both first-order-in-time (FOT) and second-order-in-time (SOT) Hermite schemes are developed. Hermite methods use the solution and multiple derivatives as unknowns and achieve space-time orders of accuracy $2m-1$ (FOT) and $2m$ (SOT) for methods using $(m+1)^d$ degree of freedom per node in $d$ dimensions. The compatibility boundary conditions (CBCs) are based on taking time derivatives of the boundary conditions and using the governing equations to replace the time derivatives with spatial derivatives. These resulting constraint equations augment the Hermite scheme on the boundary. The solvability of the equations resulting from the compatibility conditions are analyzed. Numerical examples demonstrate the accuracy and stability of the new schemes in two dimensions.

==> tex/cflLimits.tex <==

\clearpage
\section{CFL restrictions - 1D }

To test the stablity of the scheme we perform some long time simulations and look for any instabilities.
As shown in Table~\ref{tab:stableCFL1D} the ME scheme has trouble on the curvlinear grid with the tanh mapping.

\mni
Note: The code seems to first go unstable where the mesh spacing changes most rapidly.

\begin{table}[hbt]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
 \multicolumn{8}{|c|}{Stable CFL in 1D}  \\ \hline
         &     &  \multicolumn{3}{|c|}{ME}   &  \multicolumn{3}{|c|}{FOS}   \\ \hline
   BC    &  m  &  ident & tanh      & poly     &  ident & tanh    & poly   \\ \hline 
% 
    D    &  1  &   .99  &   .6      &          &  .99   &   .99   &      \\
    D    &  2  &   .99  &   .4      &          &  .99   &   .99   &      \\
    D    &  3  &   .99  &   .3      &          &  .99   &   .99   &      \\
    D    &  4  &   .99  &   .2      &          &  .99   &   .90   &      \\
    D    &  5  &   .99  &   .2      &          &  .99   &   .8    &      \\
  \hline
\end{tabular}
\caption{Experimentally found stable CFL values for various schemes and grids in one dimension.}
\label{tab:stableCFL1D}
\end{table}


\mni
Table~\ref{tab:stableCFL1DHermiteSmoothing} shows stable CFL numbers when some artificial dissipation is added.
A simple way to add dissipation is to use Hermite interpolation. At the end of a time-step, we interpolate the solution to the dual grid,
apply boundary conditions, and then interpolate back to the primal grid. This process can be repeated to give additional
smoothing. As shown in Table~\ref{tab:stableCFL1DHermiteSmoothing}, this Hermite interpolation can be used to improve the
stable CFL. At larger values of $m$, this approach is not so effective, however, and an alternative means of adding dissipation 
would seem warranted.


\begin{table}[hbt]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
    \multicolumn{8}{|c|}{Stable CFL in 1D with Hermite Smoothing}  \\ \hline
         &     &  \multicolumn{3}{|c|}{ME}   &  \multicolumn{3}{|c|}{FOS}   \\ \hline
   BC    &  m  &  ident & tanh (HS)    & poly  &  ident & tanh    &  poly  \\ \hline 
% 
    D    &  1  &   .99  &   .99 (2) &          &        &         &      \\
    D    &  2  &   .99  &   .99 (2) &          &        &         &      \\
    D    &  3  &   .99  &   .99 (4) &          &        &         &      \\
    D    &  4  &   .99  &   .9  (6) &          &        &         &      \\
    D    &  5  &   .99  &   .8 (20) &          &        &         &      \\
  \hline
\end{tabular}
\caption{Experimentally found stable CFL values with Hermite Smooths for various schemes and grids in one dimension.
  The value in parentheses is the number of Hermite smooths.
}
\label{tab:stableCFL1DHermiteSmoothing}
\end{table}


\mni
As noted by Daniel, as the mesh is refined the stable CFL should approach 1 since the lower-order terms will become less important.
Table~\ref{tab:stableCFL1DVaryingN} shows this is true for $m=3$.

\begin{table}[hbt]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
 \hline
   \multicolumn{5}{|c|}{ME: Stable CFL vs N} \\ \hline
        &  20   &  40  &   80  & 160  \\  \hline
  m=3   &  .3   &  .35 &  .4   & .95  \\
  \hline
\end{tabular}
\end{center}
\caption{Experimentally found stable CFL versus number of grid points for the tanh mapping.
}
\label{tab:stableCFL1DVaryingN}
\end{table}



\clearpage
\section{CFL restrictions - 2D }

To test the stablity of the scheme we perform some long time simulations and look for any instabilities.There is a fix to the FOT scheme in 2D to increase the stable CFL to $1$, but that fix has not been included here.

\mni
As shown in Table~\ref{tab:stableCFL2D} the ME scheme has trouble on the curvilinear grids.

\mni
Note: The code seems to first go unstable where the mesh spacing changes most rapidly.

\begin{table}[hbt]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
 \multicolumn{8}{|c|}{Stable CFL in 2D}  \\ \hline
         &     &  \multicolumn{3}{|c|}{ME}   &  \multicolumn{3}{|c|}{FOS}   \\ \hline
   BC    &  m  &  ident & tanh    & X        &  ident & tanh    & X    \\ \hline 
% 
    D    &  1  &   .99  &  .7     &          &   .85   &         &      \\
    D    &  2  &   .99  &  .3     &          &   .85   &         &      \\
    D    &  3  &   .99  &  .2     &          &   .65   &         &      \\
    D    &  4  &   .99  &  .1     &          &   .6    &         &      \\
    D    &  5  &   .99  &         &          &   .6    &         &      \\
  \hline
\end{tabular}
\caption{Experimentally found stable CFL values for various schemes and grids in two dimensions}
\label{tab:stableCFL2D}
\end{table}

\mni
Table~\ref{tab:stableCFL1DHermiteSmoothing} shows stable CFL numbers when some artificial dissipation is added.
As in 1D, the stable CFL can be increased using Hermite interpolation smoothing, but this becomes less effective
for larger values of m.

\begin{table}[hbt]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
 \multicolumn{8}{|c|}{Stable CFL in 2D with Hermite Smoothing}  \\ \hline
         &     &  \multicolumn{3}{|c|}{ME}   &  \multicolumn{3}{|c|}{FOS}   \\ \hline
   BC    &  m  &  ident & tanh      & X        &  ident  & tanh    & X    \\ \hline 
    D    &  1  &   .99  &  .99 (2)  &          &   .85   &         &      \\
    D    &  2  &   .99  &  .99 (2)  &          &   .85   &         &      \\
    D    &  3  &   .99  &  .9 (16)  &          &   .65   &         &      \\
    D    &  4  &   .99  &  .4 (8)   &          &   .6    &         &      \\
    D    &  5  &   .99  &           &          &   .6    &         &      \\
  \hline
\end{tabular}
\caption{Experimentally found stable CFL values for various schemes and grids in two dimensions with Hermite smoothing.
  The value in parentheses is the number of Hermite smooths.
}
\label{tab:stableCFL1DHermiteSmoothing}
\end{table}


% \begin{table}
% \begin{tabular}{|c|c|c|c|c|}
%  \hline
%               &  Identity         &  polynomial & tanh       & X   \\ \hline
%   ME, bc=d    &  CFL=1. (m=1:5)   &             &            &     \\ 
%   ME, bc=n    &  CFL=1. (m=1:5)   &             &            &     \\ \hline 
%   FOT, bc=d   &                   &             &            &     \\
%   FOT, bc=n   &                   &             &            &     \\
%   \hline
% \end{tabular}
% \caption{CFL bounds for various schemes and grids}
% \end{table}


==> tex/convergenceFigs.tex <==
\clearpage
\section{Convergence Figs}

% -------------------------------------------------------------------------------------------------
{
\newcommand{\figw}{5.5cm}
\newcommand{\figh}{5.5cm}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
  \useasboundingbox (0,.5) rectangle (16.5,12);  % set the bounding box (so we have less surrounding white space)

  \begin{scope}[yshift=6cm]
     \figByWidth{0.0}{0}{fig/ME2DsineBCdMapiConvergence}{\figw}[0][0][0][0];
     \figByWidth{5.5}{0}{fig/ME2DsineBCdMappConvergence}{\figw}[0][0][0][0];
     \figByWidth{11.}{0}{fig/ME2DsineBCdMapaConvergence}{\figw}[0][0][0][0];
  \end{scope} 
  \begin{scope}[yshift=0cm]
    \figByWidth{0}{0}{fig/ME2DsineBCnMapiConvergence}{\figw}[0][0][0][0];
    \figByWidth{5.5}{0}{fig/ME2DsineBCnMappConvergence}{\figw}[0][0][0][0];
     \figByWidth{11.}{0}{fig/ME2DsineBCnMapaConvergence}{\figw}[0][0][0][0];
  \end{scope}   
  % \draw[step=1cm,gray] (0,0) grid (16.5,12);
\end{tikzpicture}
\end{center}
\caption{
Grid convergence, Hermite ME scheme in 2D. 
% Left: Cartesian grid. Right: Curvilinear grid. Top: Dirichlet BC. Bottom: Neumann BC.
 }
\label{fig:hermite2DME}
\end{figure}
}

% -------------------------------------------------------------------------------------------------
{
\newcommand{\figw}{5.5cm}
\newcommand{\figh}{5.5cm}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
  \useasboundingbox (0,.5) rectangle (16.5,12);  % set the bounding box (so we have less surrounding white space)

  \begin{scope}[yshift=6cm]
     \figByWidth{0.0}{0}{fig/ME2DsineBCdMaptConvergence}{\figw}[0][0][0][0];
     \figByWidth{5.5}{0}{fig/ME2DsineBCdMaprConvergence}{\figw}[0][0][0][0];
     \figByWidth{11.}{0}{fig/ME2DsineBCdMapsConvergence}{\figw}[0][0][0][0];
  \end{scope} 
  \begin{scope}[yshift=0cm]
    \figByWidth{0}{0}{fig/ME2DsineBCnMaptConvergence}{\figw}[0][0][0][0];
    \figByWidth{5.5}{0}{fig/ME2DsineBCnMaprConvergence}{\figw}[0][0][0][0];
     \figByWidth{11.}{0}{fig/ME2DsineBCnMapsConvergence}{\figw}[0][0][0][0];
  \end{scope}   
  % \draw[step=1cm,gray] (0,0) grid (16.5,12);
\end{tikzpicture}
\end{center}
\caption{
Grid convergence, Hermite ME scheme in 2D. 
% Left: Cartesian grid. Right: Curvilinear grid. Top: Dirichlet BC. Bottom: Neumann BC.
 }
\label{fig:hermite2DME}
\end{figure}
}


% -------------------------------------------------------------------------------------------------
{
\newcommand{\figw}{5.5cm}
\newcommand{\figh}{5.5cm}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
  \useasboundingbox (0,.5) rectangle (16.5,12);  % set the bounding box (so we have less surrounding white space)

  \begin{scope}[yshift=6cm]
     \figByWidth{0.0}{0}{fig/FOT2DsineBCdMapiConvergence}{\figw}[0][0][0][0];
     \figByWidth{5.5}{0}{fig/FOT2DsineBCdMappConvergence}{\figw}[0][0][0][0];
     \figByWidth{11.}{0}{fig/FOT2DsineBCdMapaConvergence}{\figw}[0][0][0][0];
  \end{scope} 
  \begin{scope}[yshift=0cm]
    \figByWidth{0}{0}{fig/FOT2DsineBCnMapiConvergence}{\figw}[0][0][0][0];
    \figByWidth{5.5}{0}{fig/FOT2DsineBCnMappConvergence}{\figw}[0][0][0][0];
     \figByWidth{11.}{0}{fig/FOT2DsineBCnMapaConvergence}{\figw}[0][0][0][0];
  \end{scope}   
  % \draw[step=1cm,gray] (0,0) grid (16.5,12);
\end{tikzpicture}
\end{center}
\caption{
Grid convergence, Hermite FOT scheme in 2D. 
% Left: Cartesian grid. Right: Curvilinear grid. Top: Dirichlet BC. Bottom: Neumann BC.
 }
\label{fig:hermite2DFOT}
\end{figure}
}

% -------------------------------------------------------------------------------------------------
{
\newcommand{\figw}{5.5cm}
\newcommand{\figh}{5.5cm}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
  \useasboundingbox (0,.5) rectangle (16.5,12);  % set the bounding box (so we have less surrounding white space)

  \begin{scope}[yshift=6cm]
     \figByWidth{0.0}{0}{fig/FOT2DsineBCdMaptConvergence}{\figw}[0][0][0][0];
     \figByWidth{5.5}{0}{fig/FOT2DsineBCdMaprConvergence}{\figw}[0][0][0][0];
     \figByWidth{11.}{0}{fig/FOT2DsineBCdMapsConvergence}{\figw}[0][0][0][0];
  \end{scope} 
  \begin{scope}[yshift=0cm]
    \figByWidth{0}{0}{fig/FOT2DsineBCnMaptConvergence}{\figw}[0][0][0][0];
    \figByWidth{5.5}{0}{fig/FOT2DsineBCnMaprConvergence}{\figw}[0][0][0][0];
     \figByWidth{11.}{0}{fig/FOT2DsineBCnMapsConvergence}{\figw}[0][0][0][0];
  \end{scope}   
  % \draw[step=1cm,gray] (0,0) grid (16.5,12);
\end{tikzpicture}
\end{center}
\caption{
Grid convergence, Hermite FOT scheme in 2D. 
% Left: Cartesian grid. Right: Curvilinear grid. Top: Dirichlet BC. Bottom: Neumann BC.
 }
\label{fig:hermite2DFOT}
\end{figure}
}

% --------------------------------------------------------------------------
\clearpage
\section{More Convergence Tables - finer grids and higher order}

\mni
Here are some results for finer grids and $m=1,2,3,4,5$.

\mni
The errors for FOT $m=5$ on the tanh mapping saturate quite early -- need to check this out.

% -------------------------------------------------------------------------------------------------
{
\newcommand{\figw}{5.5cm}
\newcommand{\figh}{5.5cm}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
  \useasboundingbox (0,.5) rectangle (16.5,6);  % set the bounding box (so we have less surrounding white space)

  \begin{scope}[yshift=0cm]
     \figByWidth{0.0}{0}{fig/ME2DsineBCdMapim5Convergence}{\figw}[0][0][0][0];
     \figByWidth{6.5}{0}{fig/FOT2DsineBCdMaptm5Convergence}{\figw}[0][0][0][0];
     % \figByWidth{11.}{0}{fig/ME2DsineBCdMapaConvergence}{\figw}[0][0][0][0];
  \end{scope} 
  % \begin{scope}[yshift=0cm]
  %   \figByWidth{0}{0}{fig/ME2DsineBCnMapiConvergence}{\figw}[0][0][0][0];
  %   \figByWidth{5.5}{0}{fig/ME2DsineBCnMappConvergence}{\figw}[0][0][0][0];
  %    \figByWidth{11.}{0}{fig/ME2DsineBCnMapaConvergence}{\figw}[0][0][0][0];
  % \end{scope}   
  % \draw[step=1cm,gray] (0,0) grid (16.5,12);
\end{tikzpicture}
\end{center}
\caption{
Grid convergence, Hermite ME and FOT schemes in 2D. 
% Left: Cartesian grid. Right: Curvilinear grid. Top: Dirichlet BC. Bottom: Neumann BC.
 }
\label{fig:hermite2DMEV2}
\end{figure}
}


